ORCAID: Oblique Rule-Based Continuous-Action Interpretation for Deep RL Policies

Explainability remains a key issue in reinforcement learning (RL). Distilling an interpretable policy from an agent trained in a complex environment is particularly challenging when the action space is continuous. We introduce ORCAID, a novel method for extracting interpretable rule-based policies from RL agents operating in mixed continuous-discrete environments with continuous action spaces. Our main contribution is an efficient oblique decision tree training algorithm that partitions the state space by hyperplanes and fits local linear models. The key idea lies in a three-stage split search: efficient random initialization, local refinement, and backward elimination. Finally, adjacent leaves are merged to yield a concise set of interpretable rules describing a given deep RL policy. We evaluate ORCAID across multiple RL environments, demonstrating that the extracted rule-based policies maintain strong performance with a low number of parameters and can even be used to improve the performance of the original deep RL policy.

==> tables/rule_learning/DT_halfCheetah.tex <==
\begin{tabular}{|ccccccc}
\multicolumn{7}{c}{Maximum depth}  \\
 1 & 4 & 7 & 10 & 13 & 16 & 20\\\hline
 -3$\pm$0 & 20$\pm$4 & 36$\pm$4 & 45$\pm$4 & 47$\pm$4 & 47$\pm$4 & 47$\pm$4\\
 170$\pm$4 & 110$\pm$1 & 79$\pm$1 & 69$\pm$0 & 68$\pm$0 & 67$\pm$0 & 67$\pm$1\\
 170$\pm$4 & 110$\pm$1 & 82$\pm$0 & 74$\pm$0 & 72$\pm$0 & 72$\pm$0 & 72$\pm$0\\
 .04$\pm$0 & .3$\pm$.0 & 1.9$\pm$.0 & 3.6$\pm$.0 & 4.6$\pm$.0 & 5.3$\pm$.1 & 6.0$\pm$.2\\
 20$\pm$3 & 17$\pm$3 & 15$\pm$2 & 11$\pm$1 & 11$\pm$2 & 12$\pm$2 & 16$\pm$4\\
\bottomrule
\end{tabular}
\caption{Ratio between the rewards from the surrogate model and the RL policy, MSE for the training and test sets ($\times 10^{-3}$), model size, and learning time for DT for \halfCheetah.}
\label{tab:dt_hc}

==> tables/rule_learning/DT_hopper.tex <==
\begin{tabular}{|ccccccc}
\multicolumn{7}{c}{Maximum depth}  \\
 1 & 4 & 7 & 10 & 13 & 16 & 20\\\hline
 6$\pm$0 & 13$\pm$2 & 14$\pm$2 & 15$\pm$2 & 17$\pm$2 & 17$\pm$2 & 18$\pm$2\\
 111$\pm$2 & 85$\pm$2 & 64$\pm$2 & 50$\pm$1 & 45$\pm$1 & 44$\pm$1 & 44$\pm$1\\
 112$\pm$2 & 87$\pm$2 & 69$\pm$2 & 60$\pm$2 & 56$\pm$2 & 56$\pm$2 & 56$\pm$2\\
 .02$\pm$.0 & .2$\pm$.0 & 1.2$\pm$.0 & 2.6$\pm$.1 & 3.7$\pm$.1 & 4.2$\pm$.1 & 4.2$\pm$.1\\
 5$\pm$1 & 8$\pm$2 & 8$\pm$1 & 10$\pm$2 & 9$\pm$1 & 8$\pm$1 & 8$\pm$1\\
\bottomrule
\end{tabular}
\caption{Ratio between the rewards from the surrogate model and the RL policy, MSE for the training and test sets ($\times 10^{-3}$), model size, and learning time for DT for \hopper.}
\label{tab:dt_h}

==> tables/rule_learning/DT_invDoublePendulum.tex <==
\begin{tabular}{|ccccccc}
\multicolumn{7}{c}{Maximum depth}  \\
 2 & 4 & 8 & 10 & 14 & 16 & 20\\\hline
 3$\pm$1 & 5$\pm$1 & 5$\pm$0 & 5$\pm$0 & 5$\pm$0 & 5$\pm$0 & 5$\pm$0\\
 111$\pm$2 & 70$\pm$1 & 34$\pm$2 & 32$\pm$1 & 31$\pm$1 & 31$\pm$1 & 31$\pm$1\\
 112$\pm$2 & 73$\pm$2 & 44$\pm$1 & 43$\pm$1 & 42$\pm$1 & 42$\pm$1 & 42$\pm$1\\
 .04$\pm$.0 & .2$\pm$.0 & 1.7$\pm$.0 & 2.7$\pm$.0 & 3.8$\pm$.1 & 4.1$\pm$.1 & 4.6$\pm$.2\\
 1$\pm$0 & 2$\pm$0 & 2$\pm$0 & 2$\pm$0 & 2$\pm$0 & 2$\pm$0 & 2$\pm$0\\
\bottomrule
\end{tabular}
\caption{Ratio between the rewards from the surrogate model and the RL policy, MSE for the training and test sets ($\times 10^{-3}$), model size, and learning time for DT for \invDoublePendulum.}
\label{tab:dt_idp}

==> tables/rule_learning/DT_invPendulum.tex <==
\begin{tabular}{|ccccccc}
\multicolumn{7}{c}{Maximum depth}  \\
 1 & 2 & 4 & 5 & 7 & 8 & 10\\\hline
 3$\pm$0 & 10$\pm$2 & 46$\pm$4 & 52$\pm$7 & 72$\pm$11 & 85$\pm$9 & 92$\pm$8\\
 48$\pm$3 & 27$\pm$3 & 8$\pm$1 & 5$\pm$1 & 3$\pm$0 & 2$\pm$0 & 2$\pm$0\\
 50$\pm$2 & 29$\pm$3 & 10$\pm$2 & 8$\pm$1 & 7$\pm$1 & 7$\pm$1 & 7$\pm$1\\
 10$\pm$0 & 24$\pm$0 & 120$\pm$2 & 238$\pm$5 & 618$\pm$35 & 848$\pm$44 & 1311$\pm$83\\
 1$\pm$0 & 1$\pm$0 & 5$\pm$1 & 5$\pm$1 & 9$\pm$3 & 8$\pm$1 & 8$\pm$1\\
\bottomrule
\end{tabular}
\caption{Ratio between the rewards from the surrogate model and the RL policy, MSE for the training and test sets ($\times 10^{-3}$), model size, and learning time for DT for \invPendulum.}
\label{tab:dt_ip}

==> tables/rule_learning/DT_reacher.tex <==
\begin{tabular}{|ccccccc}
\multicolumn{7}{c}{Maximum depth}  \\
 1 & 4 & 7 & 10 & 13 & 16 & 20\\\hline
 29$\pm$0 & 34$\pm$1 & 50$\pm$2 & 56$\pm$1 & 56$\pm$1 & 56$\pm$1 & 56$\pm$1\\
 11$\pm$0 & 9$\pm$0 & 7$\pm$0 & 6$\pm$0 & 6$\pm$0 & 6$\pm$0 & 6$\pm$0\\
 11$\pm$0 & 9$\pm$0 & 7$\pm$0 & 7$\pm$0 & 7$\pm$0 & 7$\pm$0 & 7$\pm$0\\
 .02$\pm$.0 & .2$\pm$.0 & 1.5$\pm$.0 & 3.0$\pm$.0 & 3.3$\pm$.0 & 3.3$\pm$.0 & 3.3$\pm$.0\\
 1$\pm$0 & 1$\pm$0 & 2$\pm$0 & 2$\pm$0 & 2$\pm$0 & 2$\pm$0 & 2$\pm$0\\
\bottomrule
\end{tabular}
\caption{Ratio between the rewards from the surrogate model and the RL policy, MSE for the training and test sets ($\times 10^{-3}$), model size, and learning time for DT for \reacher.}
\label{tab:dt_r}

==> tables/rule_learning/DT_swimmer.tex <==
\begin{tabular}{|ccccccc}
\multicolumn{7}{c}{Maximum depth}  \\
 1 & 2 & 4 & 5 & 7 & 8 & 10\\\hline
13$\pm$6 & 19$\pm$11 & 72$\pm$9 & 89$\pm$2 & 91$\pm$2 & 94$\pm$1 & 95$\pm$1\\
 120$\pm$4 & 99$\pm$3 & 72$\pm$3 & 62$\pm$3 & 50$\pm$3 & 47$\pm$3 & 45$\pm$3\\
 121$\pm$5 & 100$\pm$4 & 74$\pm$4 & 67$\pm$4 & 60$\pm$4 & 59$\pm$4 & 58$\pm$4\\
 0.02$\pm$0 & 0.04$\pm$0 & 0.2$\pm$0 & 0.4$\pm$3 & 1.2$\pm$0 & 1.6$\pm$.0 & 2.4$\pm$.1\\
 21$\pm$2 & 25$\pm$3 & 17$\pm$2 & 19$\pm$3 & 21$\pm$3 & 18$\pm$2 & 22$\pm$3\\
\bottomrule
\end{tabular}
\caption{Ratio between the rewards from the surrogate model and the RL policy, MSE for the training and test sets ($\times 10^{-3}$), model size, and learning time for DT for \swimmer.}
\label{tab:dt_s}

==> tikz_config.tex <==
\usetikzlibrary{fit, positioning,shapes,shapes.arrows,arrows.meta,fit,backgrounds}
\usepackage{pgfplots}
\makeatletter
\tikzset{
    database top segment style/.style={draw},
    database middle segment style/.style={draw},
    database bottom segment style/.style={draw},
    database/.style={
        path picture={
            \path [database bottom segment style]
                (-\db@r,-0.5*\db@sh) 
                -- ++(0,-1*\db@sh) 
                arc [start angle=180, end angle=360,
                    x radius=\db@r, y radius=\db@ar*\db@r]
                -- ++(0,1*\db@sh)
                arc [start angle=360, end angle=180,
                    x radius=\db@r, y radius=\db@ar*\db@r];
            \path [database middle segment style]
                (-\db@r,0.5*\db@sh) 
                -- ++(0,-1*\db@sh) 
                arc [start angle=180, end angle=360,
                    x radius=\db@r, y radius=\db@ar*\db@r]
                -- ++(0,1*\db@sh)
                arc [start angle=360, end angle=180,
                    x radius=\db@r, y radius=\db@ar*\db@r];
            \path [database top segment style]
                (-\db@r,1.5*\db@sh) 
                -- ++(0,-1*\db@sh) 
                arc [start angle=180, end angle=360,
                    x radius=\db@r, y radius=\db@ar*\db@r]
                -- ++(0,1*\db@sh)
                arc [start angle=360, end angle=180,
                    x radius=\db@r, y radius=\db@ar*\db@r];
            \path [database top segment style]
                (0, 1.5*\db@sh) circle [x radius=\db@r, y radius=\db@ar*\db@r];
        },
        minimum width=2*\db@r + \pgflinewidth,
        minimum height=3*\db@sh + 2*\db@ar*\db@r + \pgflinewidth,
    },
    database segment height/.store in=\db@sh,
    database radius/.store in=\db@r,
    database aspect ratio/.store in=\db@ar,
    database segment height=0.1cm,
    database radius=0.25cm,
    database aspect ratio=0.35,
    database top segment/.style={
        database top segment style/.append style={#1}},
    database middle segment/.style={
        database middle segment style/.append style={#1}},
    database bottom segment/.style={
        database bottom segment style/.append style={#1}}
}
\makeatother

\pgfplotsset{every x tick label/.append style={font=\footnotesize, yshift=0.5ex}}
\pgfplotsset{every y tick label/.append style={font=\footnotesize, xshift=0.5ex}}
\pgfplotsset{every xlabel label/.append style={font=\footnotesize}}
\pgfplotsset{
    every axis x label/.append style={font=\footnotesize},
    every axis y label/.append style={font=\footnotesize},
}

\pgfplotsset{every axis legend/.append style={at={(0.1,0.5)},anchor=east,font=\scriptsize,fill=none},width=.88\columnwidth,height=.18\textheight
}
